Geometrically Higher Order Unfitted Space-Time Methods for PDEs on Moving Domains

In this paper, we propose new geometrically unfitted space-time Finite Element methods for partial differential equations posed on moving domains of higher order accuracy in space and time. As a model problem, the convection-diffusion problem on a moving domain is studied. For geometrically higher order accuracy, we apply a parametric mapping on a background space-time tensor-product mesh. Concerning discretisation in time, we consider discontinuous Galerkin, as well as related continuous (Petrov-)Galerkin and Galerkin collocation methods. For stabilisation with respect to bad cut configurations and as an extension mechanism that is required for the latter two schemes, a ghost penalty stabilisation is employed. The article puts an emphasis on the techniques that allow to achieve a robust but higher order geometry handling for smooth domains. We investigate the computational properties of the respective methods in a series of numerical experiments. These include studies in different dimensions for different polynomial degrees in space and time, validating the higher order accuracy in both variables.

==> graphics/isoparam/content.tex <==
\begin{tikzpicture}[scale=0.70]
  \begin{scope}
    \coordinate (cBB) at (2.85*2-10,4.60*2-2);
    \coordinate (cCA) at (0.70*2-10,2.15*2-2);
    \coordinate (cCB) at (4.20*2-10,2.40*2-2);

    \coordinate (cIE) at ( $(cBB) ! 0.84 ! (cCA)$ );
    \coordinate (cIB) at ( $(cBB) ! 0.23 ! (cCB)$ );
    \draw [] (cCA) -- (cCB); % -- (cCC);
    \draw [] (cBB) -- (cCB);
    \draw [] (cBB) -- (cCA);
    \draw [opacity=0.2,fill=green] (cIB) -- (cIE) -- (cCB) -- cycle;
    \draw [opacity=0.2,fill=orange] (cIE) -- (cCA) -- (cCB) -- cycle;
    \draw [fill=none,draw=black, ultra thick] (cIB) -- (cIE) -- (cCA) -- (cCB) -- cycle;
    \draw [fill=none,draw=gray, ultra thick, dashed] (cIE) -- (cCB) ;
    \draw [ultra thick, red] (cIE) -- (cIB);
  %\end{scope}
  %\begin{scope}
    \coordinate (AB) at (1.85,6.85);
    \coordinate (AC) at (4.40,6.95);
    \coordinate (AD) at (6.85,7.00);
    \coordinate (BA) at (0.00,5.10);
    \coordinate (BB) at (2.85,4.60);
    \coordinate (BC) at (5.75,4.75);
    \coordinate (BD) at (8.50,5.32);
    \coordinate (CA) at (0.70,2.15);
    \coordinate (CB) at (4.20,2.40);
    \coordinate (CC) at (7.50,2.50);
    \coordinate (DA) at (2.75,0.00);
    \coordinate (DB) at (5.55,0.20);

    \coordinate (BE) at (1.50,4.95);
    \coordinate (BF) at (4.30,4.93);
    \coordinate (BG) at (7.20,5.15);

    \coordinate (CE) at (2.55,2.55);
    \coordinate (CF) at (6.12,2.83);

    \coordinate (FA) at (0.37,3.46);
    \coordinate (FE) at (1.60,3.57);
    \coordinate (FB) at (3.53,3.50);
    \coordinate (FF) at (4.97,3.58);
    \coordinate (FC) at (6.73,3.72);
    \coordinate (FG) at (8.00,3.91);

    \coordinate (IA) at ( $(BA) ! 0.96 ! (CA)$ );
    \coordinate (IE) at ( $(BB) ! 0.84 ! (CA)$ );
    \coordinate (IB) at ( $(BB) ! 0.23 ! (CB)$ );
    \coordinate (IF) at ( $(BC) ! 0.20 ! (CB)$ );
    \coordinate (IC) at ( $(BC) ! 0.38 ! (CC)$ );
    \coordinate (IG) at ( $(BD) ! 0.70 ! (CC)$ );

    \draw [opacity=0.075,fill=white] (IA) -- (IB) -- (IF) -- (IC) -- (IG) -- (BD) -- (AD) -- (AC) -- (AB) -- (BA) -- cycle;
    \draw [opacity=0.075,fill=blue] (IA) -- (IB) -- (IF) -- (IC) -- (IG) -- (CC) -- (DB) -- (DA) -- (CA) -- cycle;

    \draw [] (AB) -- (AC) -- (AD);
    \draw [] (BA) -- (BB) -- (BC) -- (BD);
    \draw [] (CA) -- (CB) -- (CC);
    \draw [] (DA) -- (DB);

    \draw [] (BA) -- (CA) -- (DA);
    \draw [] (AB) -- (BB) -- (CB) -- (DB);
    \draw [] (AC) -- (BC) -- (CC);
    \draw [] (AD) -- (BD);

    \draw [] (AB) -- (BA);
    \draw [] (AC) -- (BB) -- (CA);
    \draw [] (AD) -- (BC) -- (CB) -- (DA);
    \draw [] (BD) -- (CC) -- (DB);

    \draw [ultra thick, red] (IA) -- (IE);
    \draw [ultra thick, red] (IE) -- (IB);
    \draw [ultra thick, red] (IB) -- (IF);
    \draw [ultra thick, red] (IF) -- (IC);
    \draw [ultra thick, red] (IC) -- (IG);

%    \node [right,scale=1.7] at (7.3,6.7) {\color{white!60!black}$\Omega_1^{\mbox{\footnotesize{}lin}}$} ;

    \node [right,scale=1.7] at (6.6,1.0) {\color{blue!60!black}$\Omega^{\mbox{\footnotesize{}lin}}$} ;

%    \node [right,scale=1.7] at (7.7,3.4) {\color{red!60!black}$\Gamma^{\mbox{\footnotesize{}lin}}$} ;


    \node [right,scale=2.5] at (9.1,4) {\color{black}$\stackrel{\Theta_h}{\longrightarrow}$} ;

    \draw [dotted, thick] (cCA) -- (CA); % -- (cCC);
    \draw [dotted, thick] (cCB) -- (CB);
    \draw [dotted, thick] (cBB) -- (BB);

    
  \end{scope}
  \begin{scope}[xshift=340]
    \coordinate (AB) at (1.85,6.85);
    \coordinate (AC) at (4.40,6.95);
    \coordinate (AD) at (6.85,7.00);
    \coordinate (BA) at (0.00,5.10);
    \coordinate (BB) at (2.85,4.60);
    \coordinate (BC) at (5.75,4.75);
    \coordinate (BD) at (8.50,5.32);
    \coordinate (CA) at (0.70,2.15);
    \coordinate (CB) at (4.20,2.40);
    \coordinate (CC) at (7.50,2.50);
    \coordinate (DA) at (2.75,0.00);
    \coordinate (DB) at (5.55,0.20);

    \coordinate (BE) at (1.50,4.95);
    \coordinate (BF) at (4.30,4.93);
    \coordinate (BG) at (7.20,5.15);

    \coordinate (CE) at (2.55,2.55);
    \coordinate (CF) at (6.12,2.83);

    \coordinate (FA) at (0.37,3.46);
    \coordinate (FE) at (1.60,3.57);
    \coordinate (FB) at (3.53,3.50);
    \coordinate (FF) at (4.97,3.58);
    \coordinate (FC) at (6.73,3.72);
    \coordinate (FG) at (8.00,3.91);

    \coordinate (IA) at ( $(BA) ! 0.96 ! (CA)$ );
    \coordinate(IAE) at (0.74,2.335);
    \coordinate (IE) at (0.84,2.46);
    \coordinate(IEB) at (2.00,3.56);
    \coordinate (IB) at ( $(BB) ! 0.23 ! (CB)$ );
    \coordinate(IBF) at (4.20,4.33);
    \coordinate (IF) at ( $(BC) ! 0.20 ! (CB)$ );
    \coordinate(IFC) at (6.13,4.15);
    \coordinate (IC) at (6.45,4.05);
    \coordinate(ICG) at (7.35,3.65);
    \coordinate (IG) at ( $(BD) ! 0.70 ! (CC)$ );


    \draw[opacity=0.075,fill=blue] 
 plot [smooth, tension=1] coordinates {(IA) (IAE) (IE) (IEB) (IB) (IBF) (IF) (IFC) (IC) (ICG) (IG)}
 (IG) -- (CC) -- (DB) -- (DA) -- (CA) -- (IA);

    \draw[opacity=0.075,fill=white] 
(BD) --
 plot [smooth, tension=1] coordinates {(IG)(ICG)(ICG)(IC)(IFC)(IF)(IBF)(IB)(IEB)(IE)(IAE)(IA)} -- (BA) -- (AB) -- (AC) -- (AD);


    \draw [] (AB) -- (AC) -- (AD);
    \draw plot [smooth, tension=1] coordinates {(BA) (BE) (BB)};
    \draw plot [smooth, tension=1] coordinates {(BB) (BF) (BC)};
    \draw plot [smooth, tension=1] coordinates {(BC) (BG) (BD)};
    \draw plot [smooth, tension=1] coordinates {(CA) (CE) (CB)};
    \draw plot [smooth, tension=1] coordinates {(CB) (CF) (CC)};
    \draw [] (DA) -- (DB);

    \draw plot [smooth, tension=1] coordinates {(BA) (FA) (CA)};
    \draw [] (CA) -- (DA);

    \draw [] (AB) -- (BB);
    \draw plot [smooth, tension=1] coordinates {(BB) (FB) (CB)};
    \draw [] (CB) -- (DB);

    \draw [] (AC) -- (BC);
    \draw plot [smooth, tension=1] coordinates {(BC) (FC) (CC)};
    \draw [] (AD) -- (BD);

    \draw [] (AB) -- (BA);
    \draw [] (AC) -- (BB);
    \draw plot [smooth, tension=1] coordinates {(BB) (FE) (CA)};
    \draw [] (AD) -- (BC);
    \draw plot [smooth, tension=1] coordinates {(BC) (FF) (CB)};
    \draw [] (CB) -- (DA);
    \draw plot [smooth, tension=1] coordinates {(BD) (FG) (CC)};
    \draw [] (CC) -- (DB);

    \draw[ultra thick, red] plot [smooth, tension=1] coordinates {(IA) (IAE) (IE)};
    \draw[ultra thick, red] plot [smooth, tension=1] coordinates {(IE) (IEB) (IB)};
    \draw[ultra thick, red] plot [smooth, tension=1] coordinates {(IB) (IBF) (IF)};
    \draw[ultra thick, red] plot [smooth, tension=1] coordinates {(IF) (IFC) (IC)};
    \draw[ultra thick, red] plot [smooth, tension=1] coordinates {(IC) (ICG) (IG)};

%    \node [right,scale=1.7] at (7.3,6.7) {\color{white!60!black}$\Omega_{1,h}$} ;

    \node [right,scale=1.7] at (6.6,1.0) {\color{blue!60!black}$\Omega_{h}$} ;

%    \node [right,scale=1.7] at (7.7,3.4) {\color{red!60!black}$\Gamma_h$} ;

  \end{scope}
  %\begin{scope}[scale=1,yshift=240,xshift=600]
  %  \node [scale=2.2] at (0,0) {\underline{interface approximation}} ;
  %\end{scope}


\end{tikzpicture}

%%% Local Variables:
%%% TeX-master: "standalone"
%%% TeX-PDF-mode: t
%%% End:


==> num_exp/nze2_table_k2.tex <==
$i_s = 1$ & DG: 10.5k - 11.3k  \par ~~$9.4 \times 10^{-2}$ \par CG: 5.89k - 5.96k  \par ~~$1.1 \times 10^{-1}$  & 10.5k - 11.3k  \par ~~$9.5 \times 10^{-2}$ \par 5.23k - 5.52k  \par ~~$1.1 \times 10^{-1}$  & 10.5k - 11.3k  \par ~~$9.5 \times 10^{-2}$ \par 5.4k - 5.25k  \par ~~$9.7 \times 10^{-2}$  & 10.5k - 11.3k  \par ~~$9.5 \times 10^{-2}$ \par 5.4k - 5.4k  \par ~~$9.4 \times 10^{-2}$  & 10.5k - 11.3k  \par ~~$9.5 \times 10^{-2}$ \par 4.70k - 5.4k  \par ~~$9.3 \times 10^{-2}$ \\[0.2cm] 
$i_s = 2$ & DG: 32.5k - 32.7k  \par ~~$1.1 \times 10^{-2}$ \par CG: 20.4k - 20.8k  \par ~~$1.2 \times 10^{-2}$  & 29.7k - 32.3k  \par ~~$1.1 \times 10^{-2}$ \par 16.0k - 17.4k  \par ~~$1.2 \times 10^{-2}$  & 28.5k - 31.5k  \par ~~$1.1 \times 10^{-2}$ \par 14.2k - 15.8k  \par ~~$1.2 \times 10^{-2}$  & 28.5k - 31.1k  \par ~~$1.1 \times 10^{-2}$ \par 12.9k - 14.6k  \par ~~$1.2 \times 10^{-2}$  & 28.5k - 30.6k  \par ~~$1.1 \times 10^{-2}$ \par 12.8k - 14.2k  \par ~~$1.1 \times 10^{-2}$ \\[0.2cm] 
$i_s = 3$ & DG: 100k - 102k  \par ~~$2.2 \times 10^{-3}$ \par CG: 71.9k - 72.9k  \par ~~$7.1 \times 10^{-3}$  & 92.2k - 93.9k  \par ~~$1.2 \times 10^{-3}$ \par 54.9k - 57.0k  \par ~~$1.4 \times 10^{-3}$  & 84.1k - 91.1k  \par ~~$1.2 \times 10^{-3}$ \par 44.7k - 47.3k  \par ~~$1.4 \times 10^{-3}$  & 81.9k - 88.9k  \par ~~$1.2 \times 10^{-3}$ \par 39.3k - 43.3k  \par ~~$1.3 \times 10^{-3}$  & 81.9k - 87.8k  \par ~~$1.2 \times 10^{-3}$ \par 37.5k - 41.3k  \par ~~$1.3 \times 10^{-3}$ \\[0.2cm] 
$i_s = 4$ & DG: 340k - 340k  \par ~~$2.3 \times 10^{-3}$ \par CG: 257k - 269k  \par ~~$7.5 \times 10^{-3}$  & 302k - 305k  \par ~~$1.9 \times 10^{-4}$ \par 190k - 196k  \par ~~$6.4 \times 10^{-4}$  & 282k - 288k  \par ~~$1.3 \times 10^{-4}$ \par 155k - 159k  \par ~~$1.6 \times 10^{-4}$  & 270k - 281k  \par ~~$1.3 \times 10^{-4}$ \par 137k - 140k  \par ~~$1.6 \times 10^{-4}$  & 267k - 277k  \par ~~$1.3 \times 10^{-4}$ \par 128k - 131k  \par ~~$1.6 \times 10^{-4}$ \\[0.2cm] 
$i_s = 5$ & DG: 1.20M - 1.20M  \par ~~$2.3 \times 10^{-3}$ \par CG: 985k - 1.2M  \par ~~$7.5 \times 10^{-3}$  & 1.6M - 1.6M  \par ~~$1.6 \times 10^{-4}$ \par 712k - 722k  \par ~~$6.4 \times 10^{-4}$  & 990k - 1.0M  \par ~~$1.9 \times 10^{-5}$ \par 569k - 576k  \par ~~$5.3 \times 10^{-5}$  & 951k - 970k  \par ~~$1.6 \times 10^{-5}$ \par 492k - 498k  \par ~~$2.0 \times 10^{-5}$  & 937k - 959k  \par ~~$1.6 \times 10^{-5}$ \par 449k - 455k  \par ~~$2.1 \times 10^{-5}$ \\[0.2cm] 


==> num_exp/nze2_table_k4.tex <==
$i_s = 1$ & DG: 261k - 284k  \par ~~$3.3 \times 10^{-2}$ \par CG: 218k - 221k  \par ~~$3.2 \times 10^{-2}$  & 261k - 284k  \par ~~$3.0 \times 10^{-2}$ \par 190k - 203k  \par ~~$3.0 \times 10^{-2}$  & 261k - 284k  \par ~~$3.0 \times 10^{-2}$ \par 182k - 191k  \par ~~$3.1 \times 10^{-2}$  & 261k - 284k  \par ~~$3.1 \times 10^{-2}$ \par 182k - 182k  \par ~~$3.3 \times 10^{-2}$  & 261k - 284k  \par ~~$3.2 \times 10^{-2}$ \par 167k - 182k  \par ~~$3.2 \times 10^{-2}$ \\[0.2cm] 
$i_s = 2$ & DG: 800k - 809k  \par ~~$8.9 \times 10^{-4}$ \par CG: 763k - 781k  \par ~~$1.1 \times 10^{-3}$  & 721k - 795k  \par ~~$4.2 \times 10^{-4}$ \par 578k - 636k  \par ~~$5.3 \times 10^{-4}$  & 686k - 771k  \par ~~$4.1 \times 10^{-4}$ \par 502k - 570k  \par ~~$4.5 \times 10^{-4}$  & 686k - 761k  \par ~~$3.8 \times 10^{-4}$ \par 449k - 521k  \par ~~$4.0 \times 10^{-4}$  & 686k - 746k  \par ~~$3.7 \times 10^{-4}$ \par 446k - 503k  \par ~~$3.9 \times 10^{-4}$ \\[0.2cm] 
$i_s = 3$ & DG: 2.46M - 2.50M  \par ~~$1.4 \times 10^{-5}$ \par CG: 2.68M - 2.73M  \par ~~$2.8 \times 10^{-5}$  & 2.21M - 2.27M  \par ~~$9.1 \times 10^{-6}$ \par 1.99M - 2.8M  \par ~~$2.3 \times 10^{-5}$  & 1.99M - 2.19M  \par ~~$8.6 \times 10^{-6}$ \par 1.57M - 1.68M  \par ~~$2.6 \times 10^{-5}$  & 1.93M - 2.12M  \par ~~$7.6 \times 10^{-6}$ \par 1.35M - 1.52M  \par ~~$1.0 \times 10^{-5}$  & 1.93M - 2.9M  \par ~~$7.4 \times 10^{-6}$ \par 1.28M - 1.43M  \par ~~$1.0 \times 10^{-5}$ \\[0.2cm] 
$i_s = 4$ & DG: 8.28M - 8.30M  \par ~~$3.9 \times 10^{-6}$ \par CG: 9.67M - 10.1M  \par ~~$1.2 \times 10^{-5}$  & 7.23M - 7.30M  \par ~~$2.1 \times 10^{-7}$ \par 6.93M - 7.16M  \par ~~$2.2 \times 10^{-6}$  & 6.66M - 6.80M  \par ~~$1.5 \times 10^{-7}$ \par 5.49M - 5.63M  \par ~~$5.1 \times 10^{-7}$  & 6.32M - 6.61M  \par ~~$1.4 \times 10^{-7}$ \par 4.75M - 4.88M  \par ~~$3.0 \times 10^{-7}$  & 6.24M - 6.51M  \par ~~$1.4 \times 10^{-7}$ \par 4.36M - 4.50M  \par ~~$2.0 \times 10^{-7}$ \\[0.2cm] 
$i_s = 5$ & DG: 29.3M - 29.3M  \par ~~$3.8 \times 10^{-6}$ \par CG: 37.0M - 38.6M  \par ~~$1.2 \times 10^{-5}$  & 25.3M - 25.3M  \par ~~$7.1 \times 10^{-8}$ \par 25.9M - 26.3M  \par ~~$1.9 \times 10^{-6}$  & 23.1M - 23.6M  \par ~~$6.3 \times 10^{-9}$ \par 20.1M - 20.3M  \par ~~$9.7 \times 10^{-8}$  & 22.0M - 22.5M  \par ~~$7.7 \times 10^{-9}$ \par 16.9M - 17.2M  \par ~~$2.2 \times 10^{-8}$  & 21.6M - 22.2M  \par ~~$3.5 \times 10^{-9}$ \par 15.2M - 15.4M  \par ~~$9.1 \times 10^{-9}$ \\[0.2cm] 

